CMetric: A Driving Behavior Measure Using Centrality Functions

We present a new measure, CMetric, to classify driver behaviors using centrality functions. Our formulation combines concepts from computational graph theory and social traffic psychology to quantify and classify the behavior of human drivers. CMetric is used to compute the probability of a vehicle executing a driving style, as well as the intensity used to execute the style. Our approach is designed for realtime autonomous driving applications, where the trajectory of each vehicle or road-agent is extracted from a video. We compute a dynamic geometric graph (DGG) based on the positions and proximity of the road-agents and centrality functions corresponding to closeness and degree. These functions are used to compute the CMetric based on style likelihood and style intensity estimates. Our approach is general and makes no assumption about traffic density, heterogeneity, or how driving behaviors change over time. We present an algorithm to compute CMetric and demonstrate its performance on real-world traffic datasets. To test the accuracy of CMetric, we introduce a new evaluation protocol (called "Time Deviation Error") that measures the difference between human prediction and the prediction made by CMetric.

==> Tables/centrality.tex <==
\begin{table}
\caption{Definition and categorization of driving behavior~\cite{sagberg2015review}. Our approach models the specific styles through various centrality functions. }
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcr}
\toprule
Global Behavior & Specific Styles & Centrality\\
\midrule
\multirow{4}{*}{Aggressive} & Overspeeding & Degree\\
 & Overtaking / Sudden Lane-Change & Closeness  \\
  & Weaving  & Closeness \\
 & Tailgating  & Eigenvector  \\
 \midrule

\multirow{2}{*}{Conservative}& Driving Slowly or uniformly  & Degree \\
 & No Lane-change  & Closeness  \\
%  & Geometric  & -  \\
%  & Random  & Strong  \\
%  \midrule

% \multirow{4}{*}{Eigenvector}& Watts-Strogatz  &   Weak \\
%  & Holme-Kim  & Strong  \\
%  & Geometric  & - \\
%  & Random  & Strong  \\
\bottomrule
\end{tabular}
}
\label{tab: behaviors}
% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
\end{table}

==> Tables/notation.tex <==
\begin{table}
  \caption{Notations used in the paper. }
  \label{tab: notation}
  \centering
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{|c|l|}
  \hline
    Symbol  & Description \\
    \hline
    $N$ & Number of vehicles\\
    % $[m]$ & \{1,2,\ldots,m\} \\
    $\vts{\cdot}$ &Absolute Value of a matrix or vector.\\
    % $\mc{I}_d$& Set of indices corresponding to non-zero entries in a vector $d$.\\
    % $A_\mc{S}$& Set of columns of $A$, indexed by elements of $\mc{S}$.\\
    % $\li_t$ & The $t^{\textrm{th}}$ Laplacian matrix in a sequence of sub-degree matrices. \\
    % $d = \textrm{dim}\li_t$ & The dimension number of rows (or columns)) of the laplacian matrix .\\
    % $\delta$ & A binary vector of length $n$ such that $\vts{\delta} \ll n$ \\
    % $U$ & Eigenvector matrix\\
    % $\Lambda$ & Diagonal matrix with eigenvalues on the diagonal.\\
    \hline
  \end{tabular}
%   }
  }
%   \vspace{-10pt}
\end{table}

